For Manifold Learning, Deep Neural Networks can be Locality Sensitive Hash Functions

It is well established that training deep neural networks gives useful representations that capture essential features of the inputs. However, these representations are poorly understood in theory and practice. In the context of supervised learning an important question is whether these representations capture features informative for classification, while filtering out non-informative noisy ones. We explore a formalization of this question by considering a generative process where each class is associated with a high-dimensional manifold and different classes define different manifolds. Under this model, each input is produced using two latent vectors: (i) a "manifold identifier" $\gamma$ and; (ii)~a "transformation parameter" $\theta$ that shifts examples along the surface of a manifold. E.g., $\gamma$ might represent a canonical image of a dog, and $\theta$ might stand for variations in pose, background or lighting. We provide theoretical and empirical evidence that neural representations can be viewed as LSH-like functions that map each input to an embedding that is a function of solely the informative $\gamma$ and invariant to $\theta$, effectively recovering the manifold identifier $\gamma$. An important consequence of this behavior is one-shot learning to unseen classes.

==> misc.tex <==
\section{A Linear Algebraic Characterization of the Local Minima of Matrix Factorization}

\begin{lemma}
\label{lem:minima-sum-frobenius-charac}
Let $W \in \mathbb{R}^{m \times d}$ and let $r = \min(m,d)$.  Let $\hat{A},\hat{B}$ be the minima of the following constrained optimization:
$$\min_{W=AB} \|A\|_F^2 + \|B\|_F^2$$ then at a local minimum there is a matrix $R$ so that if $\svd(W) = U S V^T$ then $A = U S^{1/2} R, B = R^T S^{1/2} V^T$ where $R R^T = I$. (Here if $W$ is not full rank the SVD is written by truncating $U, S, V$ in  a way where $S$ is square and full rank).
\end{lemma}
\begin{proof}
First assume $W=I$ and $A,B$ are square. Then $B = A^{-1}$. So we can write $\svd(A) = U S V^T$ and $\svd(B) = U S^{-1} V^T$ where $S$ is diagonal. Now $\|A\|_F = \|U S V^T\|_F = \|S\|_F$ as multiplying by orthonormal matrix doesn't alter Frobenius norm (Fact~\ref{fact:unitary-preserved-frobenius}). But $\|S\|_F + \|S^{-1}\|_F = \sum_i (S_{ii}^2 + 1/S_{ii}^2)$, which is minimized only when $S_{ii} = \pm 1$. So $A$ becomes orthonormal. Further note that if that is not the case then it cannot be a local minima as there is a direction of change for some $S_{ii}$ that improves the objective.

Next look at the case when $W$ may not be $I$ but is full rank and $A,B$ are square Then let $\svd(W) = U S V^T$. So $AB = USV^T$. So $S^{-1/2} U^T A B V S^{-1/2} = I$. Now since $S^{-1/2} U^T A$ and $B V S^{-1/2}$ are inverses of each other we can write their SVD as $U_2 S_2 V_2^T$ and $V_2 S_2^{-1} U_2^T$. So $A = U S^{1/2} U_2 S_2 V_2^T$ and 
$B = V_2 S_2^{-1} U_2^T S^{1/2} V^T$. SO $|B|_F = |S_2^{-1} U_2^T S^{1/2}|_F$, 
and $|A|_F = |A^T|_F = |S_2 U_2^T S^{1/2}|_F$. Let $Y = U_2^T S^{1/2}$. Then $|A|_F + |B|_F = |S_2 Y|_F + |S_2^{-1} Y|_F  
= \sum_i (S_2)_{ii}^2 |Y_{i,*}|_F^2 + (1/S_2)_{ii}^2 |Y_{i,*}|_F^2
= \sum_i ((S_2)_{ii}^2 + (1/S_2)_{ii}^2) |Y_{i,*}|_F^2
$.
This is again minimized when $(S_2)_{ii} = \pm 1$ which means $S_2$ is orthonormal. So $A = U S^{1/2} R$, and 
$B = R^T S^{1/2} V$ where $R$ is orthonormal. Again note that if this is not true then some $(S_2)_{ii}$ can be perturbed and the objective can be locally improved.

The argument continues to hold if $A,B$ are not square as the only thing that changes is that $R$ now can become rectangular (with possibly more columns than rows) but still $R R^T = I$.

If $W$ is not full rank again we can apply the above argument in the subspace where $W$ has full rank (or equivalently writing SVDs in a way where the diagonal matrix $S$ is square but $U,V$ may be rectangular but still orthogonal).
\end{proof}

\begin{corollary}
\label{cor:minima-sum-frobenius-charac}
For any convex function $O(.)$, $\min_{A,B} O(AB) + (|A|_F^2 + |B|_F^2)$ can only be at a local minimum when $A = U S^{1/2} R$ and $B = R^T S^{1/2} V^T$ for some $U U^T = I$, $R R^T = I$, $V^T V = I$
\end{corollary}
\begin{proof}
This follows from the fact that otherwise the previous lemma can be used to alter $A,B$ while keeping the product $AB$ fixed and improve the regularizer part of the objective.
\end{proof}

% \begin{lemma}
% \label{lem:minima-sum-frobenius-charac2}
% Let $W \in \mathbb{R}^{m \times d}$ and let $r = \min(m,d)$. Let $\text{svd}(W) = USV^{\top}$ where $S \in \mathbb{R}^{r \times r}$. Let $\hat{A},\hat{B}$ be the minima of the following constrained optimization:
% $$\min_{W=AB} \|A\|_F^2 + \|B\|_F^2$$
% where $A \in \mathbb{R}^{m \times p}$ and $B \in \mathbb{R}^{p \times d}$.
% Then for some semi-orthogonal matrix $R \in \mathbb{R}^{r \times p}$ such that $R^{\top}R=I$ (i.e. $R$ has orthonormal columns), we have $\hat{A} = US^{1/2}R$ and $\hat{B} = R^{\top}S^{1/2}V^{\top}$.
% \end{lemma}
% \begin{proof}
% From Lemma~\ref{lem:frobenius-nuclear-equiv-folklore} we have that $\|\hat A\|_F^2 + \|\hat B\|_F^2 = 2\|\hat A\|_F\|\hat B\|_F$ which implies that $\|\hat A\|_F = \|\hat B\|_F$.
% Note that without loss of generality since $\hat{A}\hat{B} = W$, we can assume $\hat{A}$ is of the form $US_2V_2^\top$ for some diagonal matrix $S_2$ and semi-orthogonal matrix $V_2$, and that $\hat{B}$ is of the form $U_3S_3V^\top$ for some diagonal matrix $S_3$ and semi-orthogonal matrix $U_3$.
% Now $\|\hat{A}\|_F = \|S_2\|_F$ and $\|\hat{B}\|_F = \|S_3\|_F$ (Fact~\ref{fact:unitary-preserved-frobenius}). Hence we have $\|S_2\|_F = \|S_3\|_F$. Moreover $\|S_2\|_F^2 = \|\hat{A}\|_F\|\hat{B}\|_F = \|\hat{A}\hat{B}\|_* = \Tr(S) = \|S^{1/2}\|_F^2$.
% \end{proof}



% \begin{lemma}
% Consider a linear regression setup with covariate matrix $X \in \mathbb{R}^{n \times d}$, outcome vector $y \in \mathbb{R}^n$.
% Let $X_i$ denote the $i^{th}$ column of $X$ and let $X_{-i}$ denote the matrix $X$ with the $i^{th}$ covariate (column) dropped. Let $\hat{\theta}$ denote the OLS estimate for $\theta$ when $y$ is regressed on all of $X$, let $\hat{\theta}_{-i}$ denote the OLS estimate when $y$ is regressed on $X_{-i}$. Then,
% $$X_i^{\top}\left(y - X_{-i}\hat{\theta}_{-i} \right) = 0 \iff \hat{\theta}_i = 0.$$
% \end{lemma}
% \begin{proof}
% See Partitioned regression calculations \href{http://home.cc.umanitoba.ca/~godwinrt/4042/material/part2.pdf}{here}.
% \end{proof}

\iffalse
\begin{note}
TODO: Verify that a bound on the Frobenius norm of $B$ is all that suffices for proving generalization and convergence of gradient descent and not the number of absolute dimensions of $B$.
\end{note}


\begin{note}
If we don't care about transfer learning, it might be possible to get hashing property without variance regularization. We do this by reducing the regularization coefficient on $B$ drastically so that an increase in the norm of $B$ is not penalized by the regularizer. The small amount of regularization on $B$ still left 

Q2. If our representation $g(b)$ is 100-dimensional and each one has information, can we argue that we are actually better off using (meaning $A$ puts non-zero weight) all 100 of them even when doing binary classification? Can we argue that our approach is equivalent to a max-margin classifier in the case of two manifolds?
Q3. Are we better off if our hashes are farther apart? Unclear. Yes, for binary classification.

Q4. Can we recover $b$ from $g(b)$ "easily"? Say for starters for Gaussian input $x$.
In the infinite width case, perhaps we can claim that each coordinate of $b$ is present as a separate dimension in $g(b)$. Considering the Vandermonde matrix on the $b_i$s from the different manifolds. If $b_i$s are drawn from a Gaussian distribution, then the Vandermonde matrix above should be full rank implying that the row of $b_i$s should be linearly independent of the others. Now we want to claim that this implies that $B$ is better off not zeroing out the contribution associated with $b_i$s.

Add remarks/corollaries wherever possible to indicate that results hold for soft-max or any other convex loss. Try to generalize the whole paper to work for any convex loss and not just square loss.

Similarly, nothing special about ReLU. Can have other activation functions.

Why can we add orthogonal transforms without loss of generality? Because of local minima correspondence, between the two settings. Local minima of one will correspond exactly to local minima in the other.


Notes: Add something for softmax
Add that if B is not regularized much then for train classes hashing property holds without
variance regularization
Far off b even among new manifolds will go to different hashes
Also connection to unsupervised learning where data is clustered.
is there a simple network that transforms h(b) to b
Big advantage in getting b exactly.
how to get theta.
argue that h has a low lipschitz constant. minor distortions in the input don't affect output collection of words.
\end{note}


\subsection{TODOs}
\begin{enumerate}
    \item Corollary~\ref{cor:final-repre} uses infinite length representation. Truncate it and bound the error of truncation using Taylor error estimates (will probably decay by $1/k\sqrt{k}$.
    \item For variance regularization section, add proof that the test loss will also be small. Already know that train square loss is small. Show that this generalizes and bound what the test 0-1 loss will be.
    \item Do and add experiments *
    \item Finish the Linear manifolds Section
    \item Create the 8 page version
    \item Introduction and related work
\end{enumerate}

\fi
